Types for BioAmbients

The BioAmbients calculus is a process algebra suitable for representing compartmentalization, molecular localization and movements between compartments. In this paper we enrich this calculus with a static type system classifying each ambient with group types specifying the kind of compartments in which the ambient can stay. The type system ensures that, in a well-typed process, ambients cannot be nested in a way that violates the type hierarchy. Exploiting the information given by the group types, we also extend the operational semantics of BioAmbients with rules signalling errors that may derive from undesired ambients' moves (i.e. merging incompatible tissues). Thus, the signal of errors can help the modeller to detect and locate unwanted situations that may arise in a biological system, and give practical hints on how to avoid the undesired behaviour.

==> eptcsdata.tex <==
\providecommand{\event}{E. Merelli and P. Quaglia (Eds.)\\
From Biology To Concurrency and back 2010 (FBTC'10)
}
\providecommand{\volume}{19}
\providecommand{\anno}{2010}
\providecommand{\firstpage}{103}
\providecommand{\eid}{7}

